Unveiling the Role of Message Passing in Dual-Privacy Preservation on GNNs

Graph Neural Networks (GNNs) are powerful tools for learning representations on graphs, such as social networks. However, their vulnerability to privacy inference attacks restricts their practicality, especially in high-stake domains. To address this issue, privacy-preserving GNNs have been proposed, focusing on preserving node and/or link privacy. This work takes a step back and investigates how GNNs contribute to privacy leakage. Through theoretical analysis and simulations, we identify message passing under structural bias as the core component that allows GNNs to \textit{propagate} and \textit{amplify} privacy leakage. Building upon these findings, we propose a principled privacy-preserving GNN framework that effectively safeguards both node and link privacy, referred to as dual-privacy preservation. The framework comprises three major modules: a Sensitive Information Obfuscation Module that removes sensitive information from node embeddings, a Dynamic Structure Debiasing Module that dynamically corrects the structural bias, and an Adversarial Learning Module that optimizes the privacy-utility trade-off. Experimental results on four benchmark datasets validate the effectiveness of the proposed model in protecting both node and link privacy while preserving high utility for downstream tasks, such as node classification.

==> Comments.tex <==
----------------------- \textbf{REVIEW 1} ---------------------

----------- Weaknesses -----------

W1. The paper is not well-motivated. The example in the Introduction that the attacker can infer a female user's university based on her friends on the social network does not demonstrate that such privacy leakage is enabled by the structure bias (e.g., female-female links vs. male-male links).

W2. Structure bias is not formally defined in the paper.  It should be formally defined upon some "protected attributes" (e.g., gender or race), which may not be the same as the "sensitive attributes" that are used for privacy.

W3. The threat model is very confusing. Which specific node-level and link-level privacy attacks were considered? As node-level and link-level privacy attacks were measured "by the sensitive attributes inference accuracy and link prediction accuracy" in the problem analysis (Section 3), I guess that the node-level privacy attack is indeed the attribute inference attack.  But which link-level privacy attacks do you consider? Did you consider membership inference attacks? But the attack through link prediction was too straightforward. Some state-of-the-art works on link-level membership inference attacks are listed below.
* Wu, Fan, et al. "Linkteller: Recovering private edges from graph neural networks via influence analysis." 2022 IEEE Symposium on Security and Privacy (SP). IEEE, 2022.
* Zhang, Zhikun, et al. "Inference attacks against graph neural networks." Proceedings of the 31th USENIX Security Symposium. 2022.

W4. The measurement of link-level privacy preservation should be performed through the accuracy the state-of-the-art link membership inference attacks against the proposed methods. Some state-of-the-art link membership inference attacks can be found in W3.

W5. Do the three real-world datasets used in the experiments have structural bias? There is no justification of why these 3 datasets were picked.  Also a naive method of privacy protection is to simply remove the sensitive attributes. What will be the performance of the naive method compared with DPGAL in terms of both privacy and utility?


----------- Suggestions for improvements -----------

\textbf{1. Better motivation.
2. Formalization of structural bias.
3. Formalization of threat model and attacks.
4. Have a thorough study of the existing privacy attacks against GNNs.}


----------------------- \textbf{REVIEW 2} ---------------------

----------- Weaknesses -----------
W1: Although this work provides experiments results that the proposed framework has good performance on node classification performance, it is not convincing that the proposed framework can always guarantee the privacy of nodes and links. In the current work, only the objective function of each model is provided. The authors are expected to provide a more solid theoretical analysis that the proposed model can guarantee privacy. Otherwise, empirical experiments are expected to be conducted. For instance, how will the parameters in the proposed framework affect the performance, and what is the optimal performance of the proposed framework?

W2: The details of the proposed framework are not presented well. For instance, Figure 3 provides a structure of the proposed framework. However, it seems that the SIO model is independent of other models. Additionally, the min-max game part is the core part of the proposed frameworks since it dynamically reconstructs the structure. The novelty and contribution of this model are not presented properly in the description. How will this model preserve privacy and boost utility needs to be further clarified for the audience to see the benefits of this model.

W3: This work does not provide empirical experiments on evaluating the proposed framework.

- The authors claim to preserve the utility of the model. However, to test the utility of the proposed model, only node classification experiments are conducted. Link classification experiments are also needed.

- The authors claim the proposed framework can balance the tradeoff between utility and privacy. Thus, more experiments regarding the measurement of the tradeoff between utility and privacy are needed. For instance, what parameters will have an impact on the privacy or utility needs to be discussed and presented(like testing the performance by varying different values of the privacy budget in work DPGCN).

-There are no clarifications for the comparison of existing works. Some existing works in the comparison experiments proposed to preserve privacy via local differential privacy. Other than reconstructing the structures, the value of privacy budget epsilon needs to be clarified.

----------- Suggestions for improvements -----------

1. The problem statement and problem formulation are a bit wordy. The instantiated problem description like Figure 1 is good enough. Some statements and sentences are repetitive.

2. Improve the presentation of the proposed model. The authors need to put more effort into clarifying how each model in the proposed framework does to preserve privacy and improves utility. Simply put some equations in the description of the proposed models cannot present the framework well.

3. There needs to be a more solid theoretical analysis to prove how can the proposed framework guarantee the preservation of link privacy and node privacy. Otherwise, it is not fair to compare the current works with other existing works. For instance, the DPGCN model preserves dual privacy via local differential privacy. Thus, it is for sure they can guarantee the privacy loss and control the tradeoff between privacy and utility via epsilon. Thus, the authors are expected to provide more theoretical analysis and then fix the experiments. In addition, more details of the related comparison experiments works are needed to provide such as the privacy budget for the framework.

4. There are more experiments that need to be conducted. As addressed above, more evaluation metrics are needed to test the performance of the proposed framework and other existing works, such as F1-Scores, precision, and recall. These experiments will make the effectiveness of the proposed framework more convincing.

----------------------- \textbf{REVIEW 3} ---------------------

----------- Weaknesses -----------
W1: It will be better if the authors can provide detailed discussions, theoretical analysis, or even proofs as theoretical foundation of the proposed methods. Section 5 is not very convincing. Specifically, the authors described how to do it (the implementation and design), but did not explain why to do it in the specific way described in the paper. Since it is also lacking proofs and theoretical analysis and discussions, it is also not clear if the design of the proposed approach has solid foundations.

W2: To improve the presentation, some examples can be added to explain/support the formulation of the problems and solutions. Most of the formulation part of the paper can have some simple examples to help descriptions. It is much easier to read or understand examples than reading through equations, definitions, notations, etc. (of course they are also necessary and important)

W3: The experimental evaluation can be improved by adding an evaluation of more aspects of the proposed approach. The authors provided figures of the experimental results that are intuitive. It will be better if the authors can add more insights or discussions to the experimental results in addition to the self-explained results in the figures. For example, both Sections 6.2 and 6.3 can have more discussions.

-------------------------  \textbf{METAREVIEW}  ------------------------

The main weaknesses highlighted in the reviews include:
- the problem is not well motivated
- the theoretical analysis does not seem to strongly support all the claims
- the threat model is confusing
- the experimental evaluation is not fully convincing (e.g., the choice of the datasets is not justified, and the impact of parameters on utility and performance is not analyzed)
